Automating the Correctness Assessment of AI-generated Code for Security Contexts

Evaluating the correctness of code generated by AI is a challenging open problem. In this paper, we propose a fully automated method, named ACCA, to evaluate the correctness of AI-generated code for security purposes. The method uses symbolic execution to assess whether the AI-generated code behaves as a reference implementation. We use ACCA to assess four state-of-the-art models trained to generate security-oriented assembly code and compare the results of the evaluation with different baseline solutions, including output similarity metrics, widely used in the field, and the well-known ChatGPT, the AI-powered language model developed by OpenAI. Our experiments show that our method outperforms the baseline solutions and assesses the correctness of the AI-generated code similar to the human-based evaluation, which is considered the ground truth for the assessment in the field. Moreover, ACCA has a very strong correlation with the human evaluation (Pearson's correlation coefficient r=0.84 on average). Finally, since it is a fully automated solution that does not require any human intervention, the proposed method performs the assessment of every code snippet in ~0.17s on average, which is definitely lower than the average time required by human analysts to manually inspect the code, based on our experience.

==> tex/reviewASE.tex <==
Dear Pietro Liguori,

Thank you for your submission to ASE 2023.

We are sorry to inform you that your submission #331 was not accepted for inclusion in the technical research track.

* Title: On Automated Correctness Assessment of AI Offensive Code  Generators
* Authors: Domenico Cotroneo (University of Naples Federico II);
Cristina Improta (University of Naples Federico II);
Pietro Liguori (University of Naples Federico II);
Roberto Natella (University of Naples Federico II)
* Site: https://ase2023.hotcrp.com/paper/331?cap=hcav331QGzooPUCqqGqvtRusUcehbtB

We received a record number of 629 papers (after desk rejects) this year.  Of those, 103 were accepted and 31 were accepted conditionally, yielding a likely acceptance rate of around 21%.

Below you will find the reviews along with a meta-review that summarizes the discussion that occurred after reviews were submitted to come to a consensus on your paper.

We hope that these comments can be useful in preparing your paper for submission to a future venue.

Thank you again for your interest in ASE 2023. We hope you will still be able to attend the conference in Luxembourg.

Best regards,
Federica and Chris
ASE 2023 Research Track Co-Chairs

Review #331A
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
This paper presents ASSE, a novel method for automatically evaluating the correctness of offensive shellcodes generated by AI code generators. The authors address the limitations of manual evaluation and similarity metrics by introducing symbolic execution as a means to assess the syntax and semantic correctness of AI-generated code. The authors demonstrate the effectiveness of ASSE through quantitative and correlation analysis, showing its superiority over existing metrics.

Strengths
---------
- The paper is generally well written and organized.

- The experimental results demonstrate the effectiveness of the proposed method.

Weaknesses
----------
- Weak Motivation: It is not clear if the proposed method is actually needed in practice. Also, the relationship between the proposed method and offensive code/cybersecurity is weak.

- Scalability: the method does not explicitly address scalability concerns for larger and more complex code snippets and queries.

- Partial Correctness of Code: the proposed correctness score is 0 or 1, which may not capture the potentially partial correctness of the generated code.

Comments for authors
--------------------
**Significance**: 
The problem is not well motivated. It is not clear to me how the proposed method is related to cybersecurity/offensive code. To me, it is about the general correctness of code in a specific domain. Also, it is not clear if the proposed method is actually needed in practice (if engineers will write detailed queries to generate a few lines of code, instead of writing the code directly). According to the motivating example, the query itself contains quite detailed assembly instructions. Therefore, the significance/usefulness of this work is limited.

**Novelty**:

The paper proposes to evaluate the correctness of code generated by NMT models by leveraging symbolic execution, which is new to me.

**Soundness**:

This paper proposes an automated methodology named ASSE, which leverages symbolic execution to assess the syntactic and semantic correctness of AI-generated code. The paper is generally well written. While the paper presents a potentially interesting work, there are some concerns about its soundness:

Evaluation is Limited to Short Code Snippets: According to the dataset statistics mentioned in the paper, the evaluation is primarily focused on short code snippets. This raises concerns regarding the scalability and applicability of the proposed method to more complex, larger code. Real-world applications often involve significantly more complex and extensive code. The paper would benefit from demonstrating the efficacy of ASSE on longer, more complex code snippets. The same applies to the NL queries as well.

Partial Correctness: The authors used a binary correctness score (0 or 1) in the study. However, the generated code could be partially correct.

Lack of Comparative Baseline Models: The paper currently focuses only on the evaluation of the CodeBERT model combined with a randomly initialized decoder. While this might provide some insights, it is not a comprehensive evaluation, given the absence of comparative analysis with other code generation models. Models such as CodeT5, or other state-of-the-art AI code generators, should be included in the evaluation for a well-rounded assessment. The inclusion of such models could present a broader picture of how ASSE performs across different AI code generators. Without these, the generalizability of the findings could be limited.

Unclear Settings for Human Evaluation: The human evaluation component of the study appears to lack detailed settings and guidelines. Critical information such as the number of human evaluators, their qualifications or level of expertise, and the process to reconcile differing evaluations is missing. In addition, the paper also mentions the issue of human misclassification in the “Qualitative Analysis” part, which further emphasizes the need for a more transparent evaluation process.

Limited PL/code type: The performance of this method on other types of shellcode or other programming languages is unknown. 
Verifiability and Transparency: It would be better if the authors could publicly provide the source code to ensure reproducibility.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #331B
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
This paper proposes an automatic technique, namely ASSE, for assessing the correctness of AI Offensive code generators. ASSE utilizes symbolic execution to compare the behaviors of the generated code with those of the ground truth. The paper also conducted experiments to investigate the effectiveness of ASSE. The experimental results demonstrate that ASSE outperforms similarity metrics in assessing both the syntactic and semantic correctness of the generated code and can significantly save testing time compared to human evaluation.

Strengths
---------
+ This paper is well-written.
+ The effectiveness is good from the current evaluation.

Weaknesses
----------
- The idea is not novel. - The generality of the approach is unclear.
- The evaluation subject is limited.

Comments for authors
--------------------
This work aims to improve the correctness assessment of AI generated code. The proposed approach is based on symbolic execution. Indeed, the idea is reasonable. In general, this paper is easy to follow.

This work also performs an experimental study to evaluate the proposed approach by comparing with similarity metrics. From the results, the effectiveness of the approach is demonstrated. 
However, this work has the following main problems:

First, the most critical issue lies in the novelty of this work. Leveraging symbolic execution to check semantic consistency has been proposed and used in the area of compiler validation. For example, [1] applied symbolic execution on the bytecode produced by the compilation with optimizations and that produced by the compilation without optimizations, in order to detect compiler bugs. [2] detected compiler bugs by comparing assembly language outputs through symbolic execution. The goal of using symbolic execution is also to check code semantic consistency, since compilers should preserve semantics. 
[1] Clément Béra, Eliot Miranda, Marcus Denker, and Stéphane Ducasse. 2016. Practical validation of bytecode to bytecode JIT compiler dynamic deoptimization. Journal of Object Technology (JOT) 15, 2 (2016), 1:1–26.

[2] Chris Hawblitzel, Shuvendu K. Lahiri, Kshama Pawar, Hammad Hashmi, Sedar Gokbulut, Lakshan Fernando, Dave Detlefs, and Scott Wadsworth. 2013. Will You Still Compile Me Tomorrow? Static Cross-version Compiler Validation. In Proceedings of the 2013 9th Joint Meeting on Foundations of Software Engineering. 191–201.

Second, the generality of the approach is unclear. The approach and the evaluation are presented specific to assembly code, but it is unclear whether it can be generalized to the code written in other programming languages.

Third, the evaluation is also small-scale. Only one dataset and one CodeBERT model are used in the evaluation to investigate the effectiveness and efficiency of the approach. It is unclear whether the approach can also perform well on other subjects. This is a big threat.

In particular, the subject is built by themselves. Why not use the widely-studied subjects in the area of code generation for evaluation? Also, there are many more advanced pre-trained models than CodeBERT currently. Why just considering CodeBERT?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #331C
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
This paper proposes ASSE, an automated assessing approach for the security issues in code generators. ASSE is evaluated on the code generator model with comparison to both human evaluation and similarity metrics. The results show that ASSE is able to evaluate both the syntax and semantics of the generated code in a satisfactory effectiveness.

Strengths
---------
The paper constructs a new assembly code generation dataset, which could be potentially beneficial for the future work.

Weaknesses
----------
The paper does not compare to general test generation techniques in the code assessment task, which is quite unreasonable to me since the reference implementation is given. 
The scope of the paper should be re-defined, i.e., it currently targets at assembly code generation, which is quite different from the general code generation studied in most existing work. 
The generality and scalability of the approach are unclear, i.e., the paper only considers the CodeBERT model and the scale of the assessed assembly code is not given (but I’m concerned about this part given the widely-known scalability issues in symbolic execution)

Comments for authors
--------------------
**Soundness.** My first question is why the existing test generation techniques are not included as baselines, especially the paper targets at a scenario where a reference implementation is already given. The paper claims in the related work section that “to estimate the functional correctness of a program, however, a set of unit tests needs to be manually constructed. This requires a significant effort that is often unfeasible for large amounts of generated code.”. IMHO, this claim is not true in this paper. Since the reference implementation is already given, it is intuitive to apply existing test generation techniques to generate test inputs and use the output of the reference implementation as the test oracles (which is widely known as differential testing). Therefore, it is feasible and also necessary to include test generation


The evaluation is insufficient to me, which cannot well demonstrate the soundness of the approach. 
* First, the generality of the proposed approach might be limited since the current evaluation only includes one AI code generator model (i.e., CodeBERT), which is not new and no longer the best model in the code generation task.  Since the paper aims at proposing an assessment approach, I feel that it is better to show the accuracy of the proposed approach on more than one AI code generators.

* Second, the scalability of the approach is not well discussed neither. The approach relies on the symbolic execution, which suffers from scalability issues. In particular, I fail to find the scale of the assessed assembly code, which I believe could be helpful to address my concern on the scalability issue.

**Novelty.** I think the largest novelty might be the scenario about the assembly code generation evaluation.  The detailed step in the approach is not new though.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #331D
===========================================================================

Metareview
----------
Thanks for submitting this paper to ASE! Although all the reviewers appreciate the presentation quality and good evaluation effectiveness, this paper also suffers from some major issues, including limited novelty, unclear generality and scalability, limited comparison, etc. Therefore, we cannot accept this paper. We hope these reviews are helpful to improve this paper for future publication.

Recommendation
--------------
C. Reject

==> tex/threats.tex <==
\noindent
\textbf{AI code generator:} To generate assembly code from NL descriptions, we employed a pre-trained state-of-the-art model such as CodeBERT.
We acknowledge that emerging NMT models are showing superior performance in different tasks, including code generation. However, the scope of this paper is not to improve the state-of-the-art performance in assembly code generation but to assess the ability of \approach{} in estimating offensive code correctness. 
We believe that CodeBERT fits well with the scope of the paper as it provides us with different enough and adequate numbers of code snippets to properly evaluate the proposed method. Indeed, the assembly code generated by the model is pretty balanced data (in terms of semantic correctness), which allows us to perform a fair evaluation of the metrics. 
Finally, despite CodeBERT being proposed in 2020, it is worth noticing that this model represents the state-of-the-art for several code-related tasks, such as code search and code documentation generation, and many other software engineering tasks~\cite{zhou2021assessing,DBLP:conf/msr/MashhadiH21, DBLP:conf/icse/AhmedD22,yu2022bashexplainer,zeng2022extensive}, including generation of offensive code~\cite{yang2023exploitgen,liguori2022can}.


\noindent
\textbf{Dataset:} This work addresses the specific problem of assessing the correctness of assembly code generated by AI solutions. The dataset we used in our experiments fit perfectly with the scope of this work. Indeed, to the best of our knowledge, this is the only available dataset for assembly code generation. 
Moreover, the dataset is manually curated and contains high-quality and non-ambiguous descriptions of the code (not available in larger corpora for code generation). This helped us to properly perform the human evaluation of the semantic correctness, i.e., to estimate whether the model's prediction is the correct translation of the NL description.
